Cephalometric Landmark Detection by AttentiveFeature Pyramid Fusion and Regression-Voting

Marking anatomical landmarks in cephalometric radiography is a critical operation in cephalometric analysis. Automatically and accurately locating these landmarks is a challenging issue because different landmarks require different levels of resolution and semantics. Based on this observation, we propose a novel attentive feature pyramid fusion module (AFPF) to explicitly shape high-resolution and semantically enhanced fusion features to achieve significantly higher accuracy than existing deep learning-based methods. We also combine heat maps and offset maps to perform pixel-wise regression-voting to improve detection accuracy. By incorporating the AFPF and regression-voting, we develop an end-to-end deep learning framework that improves detection accuracy by 7%~11% for all the evaluation metrics over the state-of-the-art method. We present ablation studies to give more insights into different components of our method and demonstrate its generalization capability and stability for unseen data from diverse devices.

==> back.tex <==
% =======
% table. 02
% =======
\begin{table*}[h]
    %\scriptsize
	\centering
	\caption{SUCCESSFUL DETECTION RESULTS}\label{tab:tab2}
	\begin{tabular}{|c|c|c c c c c|c c c c c|}
		\hline
		\multirow{2}*{\tabincell{c}{Network}} & \multirow{2}*{\tabincell{c}{configure}} & \multicolumn{5}{c|}{Test dataset 1} & \multicolumn{5}{c|}{Test dataset 2}\\
        \cline{3-12}
		%\multirow{2}*{\tabincell{c}{VGG19\_bn}} &  \multicolumn{10}{c|}{~}\\
		~ &~ & MRE& 2mm & 2.5mm & 3mm & 4mm & MRE & 2mm & 2.5mm & 3mm & 4mm \\
		\cline{1-12}
		%~ &VGG19\_bn &  \multicolumn{10}{c|}{~}\\
		%\cline{2-12}
		
		\multirow{4}*{\tabincell{c}{\begin{sideways}VGG19\_bn\end{sideways}}} &baseline & 2.62& 70.53 & 80.00 & 86.25 & 92.77 & 2.80 & 59.42 & 71.16 & 79.16 & 89.26 \\
		\cline{2-12} 
		~ &AFPF & 1.81& 77.37&86.67&92.24&96.39 &1.85 &66.89 &76.00 &83.16 &92.58 \\
		\cline{2-12}
		~ &~ & 1.35&83.86 &90.91 &94.21 &97.64 &1.54&73.89 &82.32 &88.00 &94.63  \\
		\cline{2-12}
		~ &~ & \textbf{1.15}&\textbf{87.12} &\textbf{92.74} &\textbf{95.93} &\textbf{98.46} &\textbf{1.46} &\textbf{74.79} &\textbf{83.68} &\textbf{88.58} &\textbf{95.47}  \\
		\cline{1-12}
		%~ &ResNet50 &  \multicolumn{10}{c|}{~}\\
		%\cline{2-12}
		\multirow{4}*{\tabincell{c}{\begin{sideways}ResNet50\end{sideways}}} &baseline & 3.16& 64.00 & 76.00 & 83.00 & 91.47 & 3.36 & 56.16 & 67.16 & 75.63 & 87.58 \\
		\cline{2-12} 
		~ &AFPF & 2.98& 66.28&77.79&85.79& 92.56 &2.89&58.05 &67.89 &77.21 &88.63 \\
		\cline{2-12}
		~ &~ & 1.40&80.74 &88.84 &93.19 &97.51 &1.63&70.05 &80.63 &86.21 &94.26  \\
		\cline{2-12}
		~ &~ & \textbf{1.18}&\textbf{86.14} &\textbf{91.72} &\textbf{95.79} &\textbf{98.25} &\textbf{1.52} &\textbf{73.37} &\textbf{81.37} &\textbf{87.53} &\textbf{94.73}  \\
		\hline
		\multirow{4}*{\tabincell{c}{\begin{sideways}Inception\end{sideways}}} &baseline & 3.16& 64.00 & 76.00 & 83.00 & 91.47 & 3.36 & 56.16 & 67.16 & 75.63 & 87.58 \\
		\cline{2-12} 
		~ &AFPF & 2.98& 66.28&77.79&85.79& 92.56 &2.89&58.05 &67.89 &77.21 &88.63 \\
		\cline{2-12}
		~ &~ & 1.40&80.74 &88.84 &93.19 &97.51 &1.63&70.05 &80.63 &86.21 &94.26  \\
		\cline{2-12}
		~ &~ & \textbf{1.18}&\textbf{86.14} &\textbf{91.72} &\textbf{95.79} &\textbf{98.25} &\textbf{1.52} &\textbf{73.37} &\textbf{81.37} &\textbf{87.53} &\textbf{94.73}  \\
		\hline
	\end{tabular}
\end{table*}

% =======
% FIG. 05
% =======
\begin{figure*}
  \centering
  \begin{center}
  \includegraphics[width=\textwidth]{photo/SDR.PNG}\\
  \caption{The successful detection rate.}\label{circuit_diagram}
  \end{center}
\end{figure*}

it is very promising for fully automated cephalometric analysis in clinical applications.
